Think before you speak: Training Language Models With Pause Tokens

Language models generate responses by producing a series of tokens in immediate succession: the $(K+1)^{th}$ token is an outcome of manipulating $K$ hidden vectors per layer, one vector per preceding token. What if instead we were to let the model manipulate say, $K+10$ hidden vectors, before it outputs the $(K+1)^{th}$ token? We operationalize this idea by performing training and inference on language models with a (learnable) $\textit{pause}$ token, a sequence of which is appended to the input prefix. We then delay extracting the model's outputs until the last pause token is seen, thereby allowing the model to process extra computation before committing to an answer. We empirically evaluate $\textit{pause-training}$ on decoder-only models of 1B and 130M parameters with causal pretraining on C4, and on downstream tasks covering reasoning, question-answering, general understanding and fact recall. Our main finding is that inference-time delays show gains when the model is both pre-trained and finetuned with delays. For the 1B model, we witness gains on 8 of 9 tasks, most prominently, a gain of $18\%$ EM score on the QA task of SQuAD, $8\%$ on CommonSenseQA and $1\%$ accuracy on the reasoning task of GSM8k. Our work raises a range of conceptual and practical future research questions on making delayed next-token prediction a widely applicable new paradigm.

==> algorithm_combined.tex <==
\begin{algorithm}[t!]
\DontPrintSemicolon

\textbf{Stage 1: Pre-training with Pause}\\
\vspace{2pt}
\hspace{10pt} \textbf{Inputs: }Pre-training dataset $\mathcal{D}_{\rm pt}$, decoder-only model $f_\theta$, number of \pausetokens $M_{\rm pt}$ to insert, pause token \pause{}\\
\vspace{2pt}

\hspace{10pt} $\textbf{p}_{[1:N]}\sim \mathcal{D}_{\rm pt}$\tcc*{\scriptsize Input Sequence from corpus}

\hspace{10pt} $\tilde{\textbf{p}}_{[1:N+M_{pt}]} = \texttt{random\_insert}(\textbf{p}_{[1:N]}, \pause{}, M_{\rm pt})$\tcc*{\scriptsize Insert $M_{\rm pt}$ pause tokens randomly in the original input sequence $\textbf{p}_{[1:N]}$, extending it's length by $M_{\rm pt}$}

\hspace{10pt} $\pauseloc = \{k \in [0, N+M_{pt}-1] \colon \tilde{p}_{k+1} = \pause{}\}$\tcc*{ \scriptsize Identify the set of positions where the next token is \texttt{<pause>}}

\hspace{10pt} $\mathcal{L}_{\rm PausePT}(f_\theta, \tilde{\mathbf{p}}_{1:N+M_{\rm pt}}) = \sum_{k=1, k\notin\pauseloc}^{N+M_{\rm pt}-1} \mathcal{L}_{\rm CE}(\tilde{p}_{k+1}, f_\theta(\tilde{\textbf{p}}_{1:k}))$ \tcc*{\scriptsize Next token prediction error excludes targets which are pause (model isn't made to learn to predict pause itself) }

\hspace{10pt}  $\theta = \theta - \nabla_\theta \mathcal{L}_{\rm PausePT}(f_\theta, \tilde{\mathbf{p}}_{1:N+M_{\rm pt}})$ \tcc*{\scriptsize Update the model}


\vspace{10pt}
\textbf{Stage 2: Fine-tuning with Pause}\\
\vspace{2pt}
\hspace{10pt} \textbf{Inputs: }Downstream labeled dataset $\mathcal{D}_{\rm ft}$, pre-trained model $f_\theta$, number of \pausetokens $M_{\text{ft}}$ to insert, pause token \pause{} \\
\vspace{2pt}
\hspace{10pt} $\textbf{p}_{[1:N]}, \textbf{t}_{[1:T]}\sim \mathcal{D}_{\rm ft}$\tcc*{\scriptsize Sample prefix and target} 

\hspace{10pt}  $\tilde{\textbf{p}}_{[1:N+M_{\text{ft}}]} = \text{Concat}([\textbf{p}_{[1:N]}, [\pause{}] \times M_{\text{ft}})$\tcc*{\scriptsize Append prefix and $M_{\rm ft}$ pauses} 

\hspace{10pt} $\mathcal{L}_{\rm PauseFT}(f_\theta, \tilde{\textbf{p}}_{[1:N+M_{\text{ft}}]}, \textbf{t}_{1:T}) = \sum_{k=0}^{T-1} \mathcal{L}_{\text{CE}}(t_{k+1}, f_\theta(\text{Concat}[\tilde{\textbf{p}}_{[1:N+M_{\rm ft}]}, \textbf{t}_{1:k}])$ \tcc*{\scriptsize Next token prediction error on targets}
\hspace{10pt}  $\theta = \theta - \nabla \mathcal{L}_{\rm PauseFT}(f_\theta, \tilde{\textbf{p}}_{[1:N+M_{\text{ft}}]}, \textbf{t}_{1:T})$ 

\vspace{10pt}
\textbf{Stage 3: Inference with Pause}\\
\vspace{2pt}
\hspace{10pt} \textbf{Inputs: }Prefix $\textbf{p}_{[1:N]}$, fine-tuned model $f_\theta$, number of \pausetokens $M_{\text{inf}}$ to insert, Pause token \pause{} \\
\vspace{2pt}
\hspace{10pt} $\tilde{\textbf{p}}_{[1:N+M_{\text{inf}}]} = \text{Concat}([\textbf{p}_{[1:N]}, [\pause{}] \times M_{\text{inf}}])$\tcc*{\scriptsize Append $M_{\rm inf}$ pauses to prefix} 

\hspace{10pt}  $\tilde{\textbf{p}}_{N+M_{\text{inf}}+1} \sim f_\theta(\tilde{\textbf{p}}_{[1:N+M_{\text{inf}}]})$ \tcc*{\scriptsize Predict the next token in the sequence, and continue in an auto-regressive fashion}

\caption{Learning and Inference with Pause Tokens. Stage 1 and Stage 2 can be used independently as well, as studied in pause-training variants.}
\label{alg:main}
\end{algorithm}


==> flops_bkp.tex <==
\clearpage 
\section{Comparing FLOPS}

\textit{Floating Point Operations per Second (FLOPS)} is a critical deployment time constraint for machine learning models, especially under resource constrained environments. In this section, we compare the additional FLOPS 
in computational tasks, especially in the fields of machine learning and computer vision. It quantifies the computational capabilities of algorithms and systems, providing a benchmark for efficiency and performance. FLOPS is particularly relevant when assessing the computational cost of operations in high-dimensional data processing, which is commonplace in deep learning models. Understanding the FLOPS involved in fundamental operations allows for a more nuanced analysis of the overall computational efficiency and feasibility of various algorithms.

\begin{lemma}
\label{lemma:basic-flops}
The number of flops required to compute:
\begin{enumerate}
    \item  the dot product $\mathbf{v}_1 \cdot \mathbf{v}_2$ where $\mathbf{v}_1, \mathbf{v}_2 \in \mathbb{R}^{d}$ is 2d-1.
    \item the matrix multiplication is $M_1\cdot M_2$, where $M_1 \in
    \mathbb{R}^{a \times b}$ and $M_2 \in \mathbb{R}^{b \times c}$, the \flops is given by $a\times b\times c$.
\end{enumerate}

\end{lemma}


\begin{proof}
For a dot product between $\mathbf{v}_1$ and $\mathbf{v}_2$, both of dimension $d$, the total number of \flops  is given by the sum of multiplications and additions required. Specifically, it involves $d$ multiplications and $d - 1$ additions, totaling to $2d - 1$ FLOPS. For the ease of calculation, we approximate this as $2d$.

For a matrix multiplication of $M_1 \in \mathbb{R}^{a \times b}$ and $M_2 \in \mathbb{R}^{b \times c}$,  each element of the resulting matrix is computed by taking the dot product of a row from $M_1$ and a column from $M_2$, which requires $2b$ \flops. Since there are $a \times c$ such dot products to compute for the entire matrix multiplication, the total FLOPS amount to $(2b) \times a \times c$. However, for simplicity, if we only consider the multiplicative operations, the FLOPS reduce to $a \times b \times c$.
\end{proof}


\begin{lemma}
Let $a$ be number of multi attention heads, h be embedding dimension, 4h be hidden dimension and L be layers. 
Then 


\begin{equation}
    F(n,h,a,l) = (4anh^2 + 2an^2h + 8nh^2)\times l
\end{equation} %


\end{lemma}

\begin{proof}
\todovn{Please write these in full sentences like in a paper.}

\textbf{1. Q,K,V computation for each token} : 
Each Q,K,V is a matrix of $h\times h$ dimension and multiplied by token embedding of size $h$. And this happend for n tokens.
FLOPS = $3ah^2n$

\textbf{2. Attention mechanism} : 
we have Query matrix of $R^{n\times h}$ and K matrix of $R^{n \times h}$. So $Q^{T}$K incurs FLOPS = $n^2h$. The received scalar weights ($\alpha \in R^{n \times n}$) are then multiplied to each of the value vectors($\R^{n\times h}$), incurring $n^2h$ flops. 
Total FLOPS = $2n^2ha$.

\textbf{3. Combine MHA}: The value vectors from each head is concatenated and projected back to hidden dim. 
FLOPS = $ah^2n$

\textbf{4. Feed forward FLOPS} h $\rightarrow$ 4h and 4h$\rightarrow$ h gives FLOPS = $4h^2+4h^2=8h^2n$FLOPS.


\end{proof}

\todovn{Make a note about softmax?}


\begin{theorem}
Under the assumption $n \ll h$, the increase in FLOPS due to $p$ pause tokens is less than the increase in FLOPS due to 1 additional transformer layer, if $n > pL$.
\end{theorem}

\begin{proof}
Increase in FLOPS due to 1 additional transformer layer is give by:
\begin{align}
    F_{\Delta l=1} &= F(n,h,a,l+1)-F(n,h,a,l) \notag\\
    F_{\Delta l=1} &=4anh^2 + 2an^2h + 8nh^2
\end{align}

Similarly, increase in FLOPS due to $p$ pause tokens is given by:
\begin{align}
    F_{\Delta n=p} &= F(n+P,h,a,l)-F(n,h,a,l) \notag\\
    F_{\Delta n=p} &=(4ah + 4an + 2ap + 8h)hpl
\end{align}
Now,
\begin{align}
    F_{\Delta n=p} &< F_{\Delta l=1}\notag\\
    \implies (4ah + 4an + 2ap + 8h)hpl &< (4ah+2an+8h)nh \notag\\
    \implies (4a(n+h) + 8h + 2ap)pl &< (2an + 4ah + 8h)n\notag\\
    \implies n > &\frac{(4a+8)h + 4an + 2ap}{(4a+8)h + 2an} \cdot pl
\end{align}
Case A: $n\sim h$, we have:
\begin{align}
    n &> \frac{(8a+8)h + 2ap}{(6a+8)h} \cdot pl\notag\\
    n &> \frac{(8a+8)h + 2ap}{(6a+8)h} \cdot pl
\end{align}

Case B: $n,p<< h$, we have:
\begin{align}
    n &> pl
\end{align}
\end{proof}

\begin{theorem}
The increase in FLOPS due to $p$ pause tokens is less than the increase in FLOPS due to 1 additional attention head, if $n>\frac{4}{3}ap$.
\end{theorem}
\begin{proof}
Increase in FLOPS due to 1 additional attention head is given by:
\begin{align}
    F_{\Delta a=1} &= F(n,h,a+1,l)-F(n,h,a,l) \notag\\
    F_{\Delta a=1} &=(4nh^2 + 2n^2h)l
\end{align}
Now,
\begin{align}
    F_{\Delta n=p} &< F_{\Delta a=1}\notag\\
    \implies (4ah + 4an + 2ap + 8h)hpl &< (4nh^2 + 2n^2h)l\notag\\
    \implies ((2a+4)h + 2an + ap)p &< (2h + n)n\notag\\
    \implies n > \frac{(2a+4)h + 2an + ap}{2h+n}\cdot p
\end{align}
Case A: Assuming, $n,p<<h$, we have:
\begin{align}
    n > \frac{(2a+4)h}{2h}\cdot p\notag \\
    n > (a+2)\cdot p
\end{align}

Case B: Assuming, $n\sim h$ and $p<<h$, we have:
\begin{align}
    n > \frac{(4a+4)h}{3h}\cdot p\notag \\
    n > \frac{4}{3}(a+1)\cdot p
\end{align}
\end{proof}

\begin{theorem}
The increase in FLOPS due to $p$ pause tokens is less than the increase in FLOPS if the embedding dimension is increased by k, if $p>\frac{2nk}{h}$.
\end{theorem}

\begin{proof}
Increase in FLOPS if the embedding dimension is increased by k:
\begin{align}
    F_{\Delta h=k} &= F(n,h+k,a,l)-F(n,h,a,l) \notag\\
    F_{\Delta h=k} &=(4an((h+k)^2-h^2) + 2an^2k + 8n((h+k)^2-h^2))l\notag\\
    F_{\Delta h=k} &=(2a(2h+k) + an + 4(2h+k))2nkl\notag\\
\end{align}
Now, assuming that $k<<h$, we have:
\begin{align}
    F_{\Delta n=p} &< F_{\Delta h=k}\notag\\
    \implies (4ah + 4an + 2ap + 8h)hpl &< (4ah + an + 8h)2nkl\notag\\
    \implies ((2a+4)h + 2an + ap)hp &< ((4a+8)h + an)nk\notag\\
    \implies p &< \frac{(4a+8)h + an}{((2a+4)h + 2an + ap)}\frac{nk}{h}
\end{align}

Case A: $n,p<<h$, we have:
\begin{align}
    \implies p &< \frac{2nk}{h}
\end{align}
\end{proof}

\section{Additional parameters comparison}
\todovn{Doesn't make sense to have a whole new section for this one sentence. We should have a bullet of points stating the ways in which pause tokens are better. In FLOPS, or in wall clock time, or flexibility, or parameter count.}

Adding a new attention head is : adding a new $W_{out}^h$ matrix (see Equation 4), which is $\R^{h \times h}$. So in total new parameters per attention head is $lh^2$, which is way more than simple $ph$ new parameters for adding $p$ pause tokens



